CSCO: Connectivity Search of Convolutional Operators

Exploring dense connectivity of convolutional operators establishes critical "synapses" to communicate feature vectors from different levels and enriches the set of transformations on Computer Vision applications. Yet, even with heavy-machinery approaches such as Neural Architecture Search (NAS), discovering effective connectivity patterns requires tremendous efforts due to either constrained connectivity design space or a sub-optimal exploration process induced by an unconstrained search space. In this paper, we propose CSCO, a novel paradigm that fabricates effective connectivity of convolutional operators with minimal utilization of existing design motifs and further utilizes the discovered wiring to construct high-performing ConvNets. CSCO guides the exploration via a neural predictor as a surrogate of the ground-truth performance. We introduce Graph Isomorphism as data augmentation to improve sample efficiency and propose a Metropolis-Hastings Evolutionary Search (MH-ES) to evade locally optimal architectures and advance search quality. Results on ImageNet show ~0.6% performance improvement over hand-crafted and NAS-crafted dense connectivity. Our code is publicly available.

==> _txt/9_Checklist.tex <==
\section{Reproducibility Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} This paper proposes a new paradigm to address structural wiring of building operators in CNN architecture design.
  \item Did you describe the limitations of your work?
    \answerYes{} The only limitation is its generic applicability towards applications other than Computer Vision. We leave this as part of our future work.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{} There are no negative societal impacts.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} All authors have a clear understanding of the ethics review guidelines and try their best to follow these guidelines.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{} No theoretical results are involved in this paper.
	\item Did you include complete proofs of all theoretical results?
    \answerNA{} No theoretical results are involved in this paper.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} Please see supplementary material for more details. We release the code and/or models on CIFAR-10 for easy reproduction, and will release more demanding experimental results on ImageNet upon acceptance of this paper.
    \item Did you include the raw results of running the given instructions on the given code and data?
    \answerYes{}, see the submitted code snippet.
    \item Did you include scripts and commands that can be used to generate the figures and tables in your paper based on the raw results of the code, data, and instructions given?
    %
   \answerYes{}, see the submitted code snippet.
   \item Did you ensure sufficient code quality such that your code can be safely
    executed and the code is properly documented?
    %
    \answerYes{}, see the submitted code snippet.
    \item Did you specify all the training details (e.g., data splits,
    pre-processing, search spaces, fixed hyperparameter settings, and how they
    were chosen)?
    %
    \answerYes{} Please see main paper context on ImageNet experiments, and see Supplementary for CIFAR-10 experiments.
    %
  \item Did you ensure that you compared different methods (including your own)
    exactly on the same benchmarks, including the same datasets, search space,
    code for training and hyperparameters for that code?
    %
    \answerYes{}.
    %
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    %
    \answerYes{}, see Section 4 for comparisons that demonstrate the effectiveness of Graph Augmentation and Metropolis-Hastings Evolutionary Search.
    %
  \item Did you use the same evaluation protocol for the methods being compared?
    %
    \answerYes{}. All CIFAR-10 and ImageNet experiments are using the same training protocols as existing works.
    %
  \item Did you compare performance over time?
    %
    \answerYes{}. Please see table 4 for performance of MH-ES versus other search algorithms over time. 
    %
  \item Did you perform multiple runs of your experiments and report random seeds?
    %
    \answerYes{}. We perform multiple rounds of evaluation for Metropolis-Hastings Evolutionary Search to demonstrate its effectiveness over other search algorithms. We run end-to-end search process on CIFAR-10 multiple times and report its variance under 100-epoch training pipeline.
    %
  \item Did you report error bars (e.g., with respect to the random seed after
    running experiments multiple times)?
    %
    \answerYes{}. For CIFAR-10, we perform multiple evaluations and provide standard deviation in Supplementary Material.
    %
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    %
    \answerNA{}. Not applicable for this work.
    %
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    %
    \answerYes{}. Please see supplementary material.
    %
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML
    method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    %
    \answerYes{}, please see supplementary material for more details.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We cite both CIFAR-10 and ImageNet paper.
  \item Did you mention the license of the assets?
    \answerNA{} All assets are publicly available.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{} All assets are publicly available.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} All assets are publicly available.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} All assets are publicly available.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} Not relevant.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}. Not available for the participants in this work.
\end{enumerate}
\end{enumerate}

